On the ubiquity of duopolies in constant sum congestion games

We analyse a coalition formation game between strategic service providers of a congestible service. The key novelty of our formulation is that it is a constant sum game, i.e., the total payoff across all service providers (or coalitions of providers) is fixed, and dictated by the size of the market. The game thus captures the tension between resource pooling (to benefit from the resulting statistical economies of scale) and competition between coalitions over market share. In a departure from the prior literature on resource pooling for congestible services, we show that the grand coalition is in general not stable, once we allow for competition over market share. In fact, under classical notions of stability (defined via blocking by any coalition), we show that no partition is stable. This motivates us to introduce more restricted (and relevant) notions of blocking; interestingly, we find that the stable configurations under these novel notions of stability are duopolies, where the dominant coalition exploits its economies of scale to corner a disproportionate market share. Furthermore, we completely characterise the stable duopolies in heavy and light traffic regimes.

==> non_constant.tex <==
\section{Another Variant}
In this section, we consider another variant of the problem where the arriving customer stream still split amongst various (coalitions of) service providers according to the Wardrop Equilibrium, WE (such that the blocking probability $B$ of each coalition of service provider is same). But the utility of each coalition is now proportional to the actual customers served ($\lambda_C^\P (1-B^{WE})$) instead of the market share obtained ($\lambda_C^\P$).

In this context, our aim again is to study the partitions that are stable the three rules defined in the previous sections, i.e., GB-PA, RB-PA and RB-IA rules. 
Observe that it is not anymore clear that the worst utility of any coalition is obtained under the partition when all other players come together to form a coalition. This is because under the above mentioned arrangement of players the blocking probability at WE, $B^{WE}$ is the minimum.

We begin on similar lines as before; our first result is that all configurations involving partitions of size two or more are unstable under all the three rules.

\begin{theorem}
Under the GB-PA/RB-PA/RB-IA rules, any configuration $(\P,\Phi)$ with $|\P| \ge 2$ is not stable.
\end{theorem}
\textbf{Proof:} Consider any partition with $k \ge 2$ coalitions. Then, at WE the blocking probability of each coalition is given by $B_k.$ Next, consider the merger of any two coalitions in the partition (leading to a $(k-1)$ partition). We know that the blocking probability at the new WE is smaller than $B_k$ for the merged coalition. Further, it obtains higher market share at the new WE. Thus, the payoff of the merged coalition is greater than the sum of the payoffs of the (previous) original coalitions and hence the result follows.  \Halmos

Thus, we are only left with the possibility of grand coalition ($\P_G$) being stable for some configuration(s).
